How Do Expectations Affect Learning About Fundamentals? Some Experimental Evidence

We test how individuals with incorrect beliefs about their ability learn about an external parameter (`fundamental') when they cannot separately identify the effects of their ability, actions, and the parameter on their output. Heidhues et al. (2018) argue that learning makes overconfident individuals worse off as their beliefs about the fundamental get less accurate, causing them to take worse actions. In our experiment, subjects take incorrectly-marked tests, and we measure how they learn about the marker's accuracy over time. Overconfident subjects put in less effort, and their beliefs about the marker's accuracy got worse, as they learnt. Beliefs about the proportion of correct answers marked as correct fell by 0.05 over the experiment. We find no effect in underconfident subjects.

==> table3.tex <==
\begin{tabular}{l c c c}
\toprule
\toprule % Top horizontal line
& Fixed Effects: & Fixed Effects:
\\
&Accuracy of Marker - &Variance of Beliefs\\ 
&Overconfident Subjects& Around True $\phi$ - \\
& &Underconfident Subjects\\
\cmidrule(l){2-3}
&(1)&(2)\\
\midrule
Round& $-0.0029$& $-0.0030$ \\
& ($0.0045$)&($0.0089$)\\[1ex]
Observations&$745$&$200$\\
$R^{2}$ &$0.0009$& $0.0010$\\
\bottomrule % Bottom horizontal line
\addlinespace[1ex]
\end{tabular}
